TTSDS -- Text-to-Speech Distribution Score

Many recently published Text-to-Speech (TTS) systems produce audio close to real speech. However, TTS evaluation needs to be revisited to make sense of the results obtained with the new architectures, approaches and datasets. We propose evaluating the quality of synthetic speech as a combination of multiple factors such as prosody, speaker identity, and intelligibility. Our approach assesses how well synthetic speech mirrors real speech by obtaining correlates of each factor and measuring their distance from both real speech datasets and noise datasets. We benchmark 35 TTS systems developed between 2008 and 2024 and show that our score computed as an unweighted average of factors strongly correlates with the human evaluations from each time period.

==> other/features.tex <==
\tikzset{
    my node/.style={
        draw=gray,
        fill=gray!5,
        thick,
        minimum width=1em,
        rounded corners=3,
        font=\sffamily\footnotesize,
    }
}
\forestset{
    direction switch/.style={
        forked edges,
        for tree={
            my node,
            grow=0,
            edge+=thick, 
            font=\strut\footnotesize\sffamily,
            l sep=8pt,
            l=5pt,
        },
        where level=0{anchor=west, calign=center}{},
        where level=1{
            minimum width=5em,
            parent anchor=east, 
            calign=child edge
        }{},
        where level=2{
            minimum width=10em,
        }{},
        where level=3{
            fill=none, 
            draw=none, 
            calign=first,
            inner ysep=-2em,
        }{},
        where level>=2{
            folder, 
            grow'=0,
            s=-1em,
            s sep=-1em,
        }{},
    },
}

\begin{figure}[htb]
  \centering 
\begin{forest}
    direction switch
    [TTSDS Score,font=\strut\footnotesize\sffamily\em
        [General
            [SSL Representations
                [Hubert \cite{hsu2021hubert}]
                [wav2vec 2.0 \cite{baevski2020wav2vec2}]
            ]
        ]
        [Intelligibility
            [ASR WER
                [wav2vec 2.0 \cite{baevski2020wav2vec2}]
                [Whisper \cite{radford2023whisper}]
            ]
        ]
        [Prosody, calign=midpoint
            [SSL Representations
                [MPM \cite{mpm}]
            ]
            [Pitch
                [WORLD \cite{morise2016world}]
            ]
            [Segmental Length
                [Hubert \cite{hsu2021hubert} token length]
            ]
        ]
        [Speaker
            [Speaker Embedding
                [WeSpeaker \cite{wang2023wespeaker}]
                [DVector \cite{wan2018dvec}]
            ]
        ]
        [Environment
            [Noise/Artifacts
                [VoiceFixer \cite{liu2021voicefixer} + PESQ \cite{rix2001pesq}]
                [WADA SNR \cite{kim2008wada}]
            ]
        ]
    ]
\end{forest}
\vspace{-1em}
\caption{Features used in the benchmark and their respective factors.
%\ondrej{this would be better as a table. In intelligibility you probably meant Whisper instead of Hubert.}
}\label{fig:features}
\end{figure}
